Applications of antenna-level buffering

The purpose of this document is to discuss applications of the antenna-level buffering capability being implemented in SKA-LOW. In addition to their scientific motivation -- to detect and study cosmic rays interacting in the atmosphere -- these buffers provide access to low-level data for engineering and development work. Experience has shown that antenna-level buffered data can assist with antenna calibration, localising RFI, and diagnosing fundamental hardware problems. In this document, we describe several of these applications, with close reference to experience with LOFAR, ACTA, Parkes, and the OVRO-LWA.

==> journals.tex <==
% List of journal abbreviations.  Includes everything from the MNRAS guide, plus additions.

\newcommand{\aap}{A\&A}                  % Astronomy and Astrophysics
\newcommand{\aapr}{A\&A Rev.}            % Astronomy and Astrophysics Reviews
\newcommand{\aaps}{A\&AS}                % Astronomy and Astrophysics, Supplement
\newcommand{\aas}{AAS Abs.}              % American Astronomical Society Meeting Abstracts
\newcommand{\actaa}{Acta Astron.}        % Acta Astronomica
\newcommand{\afz}{Afz}                   % Astrofizika
\newcommand{\aipcs}{AIP Conf.\ Series}   % American Institute of Physics Conference Series
\newcommand{\aj}{AJ}                     % The Astronomical Journal
\newcommand{\aujph}{Australian J.\ Phys.} % Australian Journal of Physics
\newcommand{\astl}{Astro.\ Lett.}        % Astronomy Letters
\newcommand{\anchem}{Analytical Chem.}   % Analytical Chemistry
\newcommand{\ao}{Applied Optics}         % Applied Optics
\newcommand{\apj}{ApJ}                   % The Astrophysical Journal
\newcommand{\apjl}{ApJ Lett.}            % The Astrophysical Journal Letters
\newcommand{\apjs}{ApJS}                 % The Astrophysical Journal Supplement Series
\newcommand{\aplett}{Astrophys.\ Lett.}  % Astrophysics Letters
\newcommand{\app}{Astropart.\ Phys.}     % Astroparticle Physics
\newcommand{\apspr}{Astrophys.\ Space Phys.\ Res.} % Astrophysics Space Physics Research
\newcommand{\apss}{Ap\&SS}               % Astrophysics and Space Science
\newcommand{\apssproc}{Ap\&SS\ Proc.}    % Astrophysics and Space Science Proceedings
\newcommand{\araa}{ARA\&A}               % Annual Review of Astronomy and Astrophysics
\newcommand{\arep}{Astron.\ Rep.}        % Astronomy Reports
\newcommand{\arnps}{Annu.\ Rev.\ Nucl.\ Part.\ Sci.} % Annual Review of Nuclear and Particle Science
\newcommand{\arxiv}{arXiv}               % ArXiv
\newcommand{\aspacer}{Adv.\ Space Res.}  % Advances in Space Research
\newcommand{\aspc}{ASP Conf.\ Ser.}      % Astronomical Society of the Pacific Conference Series
\newcommand{\atel}{ATel}                 % Astronomer's Telegram
\newcommand{\azh}{AZh}                   % Astronomiceskii Zhurnal
\newcommand{\baas}{BAAS}                 % Bulletin of the American Astronomical Society
\newcommand{\bac}{Bull.\ Astron.\ Inst.\ Czechoslovakia} % Bulletin of the Astronomical Institutes of Czechoslovakia
\newcommand{\bain}{Bull.\ Astron.\ Inst.\ Netherlands} % Bulletin of the Astronomical Institute of the Netherlands
\newcommand{\bell}{Bell Systems Tech.\ J.} % Bell Systems Technical Journal
\newcommand{\caa}{Chinese Astron.\ Astrophys.} % Chinese Astronomy and Astrophysics
\newcommand{\cjaa}{Chinese J.\ Astron.\ Astrophys.} % Chinese Journal of Astronomy and Astrophysics
\newcommand{\cpc}{Comput.\ Phys.\ Commun.} % Computer Physics Communications
\newcommand{\cphysc}{Chinese Phys.~C}   % Chinese Physics C
\newcommand{\cqgrav}{Class.\ Quant.\ Grav.} % Classical and Quantum Gravity
\newcommand{\crp}{Compt.\ Rend.\ Phys.}  % Comptes Rendus Physique
\newcommand{\cosres}{Cosm.\ Res.}        % Cosmic Research
\newcommand{\dans}{Dokl.\ Akad.\ Nauk SSSR} % Doklady Akademii Nauk SSSR (some old Russian journal)
\newcommand{\dokphys}{Dokl.\ Phys.}      % Doklady Physics: English translation of Doklady Akademii Nauk
\newcommand{\dps}{AAS Plan.\ Sci.\ Abs.} % American Astronomical Society/Division for Planetary Sciences Meeting Abstracts
\newcommand{\easconf}{EAS Pub.\ Series}  % European Astronomical Society Publications Series
\newcommand{\elec}{Electronics}          % Electronics (magazine)
\newcommand{\epjc}{Eur.\ Phys.\ J.~C}    % European Physical Journal C
\newcommand{\epjwoc}{EPJ Web of Conf.}   % European Physical Journal Web of Conferences
\newcommand{\epsl}{Earth and Plan.\ Sci.\ Lett.} % Earth and Planetary Science Letters
\newcommand{\expa}{Exp.\ Astron.}        % Experimental Astronomy
\newcommand{\fcp}{Fundamentals Cosmic Phys.} % Fundamentals of Cosmic Physics
\newcommand{\fphys}{Frontiers of Physics} % Frontiers of Physics
\newcommand{\gca}{Geochimica Cosmochimica Acta} % Geochimica et Cosmochimica Acta
\newcommand{\geoji}{Geophys.\ J.\ Int'l} % Geophysical Journal International
\newcommand{\grl}{Geophys.\ Res.\ Lett.} % Geophysical Research Letters
\newcommand{\iaj}{Irish Astro.\ J.}      % Irish Astronomical Journal
\newcommand{\iaucirc}{IAU Circ.}         % International Astronomical Union Circulars
\newcommand{\iauproc}{Proc.\ IAU}        % Proceedings of the International Astronomical Union
\newcommand{\ibvs}{IBVS}                 % International Bulletin of Variable Stars
\newcommand{\icarus}{Icarus}             % Icarus
\newcommand{\ieeetit}{IEEE Trans.\ Info.\ Theor.} % IEEE Transactions on Information Theory
\newcommand{\ieeetns}{IEEE Trans.\ Nucl.\ Sci.} % IEEE Transactions on Nuclear Science
\newcommand{\ieeemtt}{IEEE Trans.\ Microwave Theor.\ \& Techniques} % IEEE Transactions on Microwave Theory and Techniques
\newcommand{\ieeemi}{IEEE Trans.\ Med.\ Imaging} % IEEE Transactions on Medical Imaging
\newcommand{\ieeeproc}{Proc.\ IEEE}      % Proceedings of the IEEE
\newcommand{\ijmpd}{Int'l J.\ Mod.\ Phys.~D} % International Journal of Modern Physics D
\newcommand{\incimento}{Nuovo Cimento} % Il Nuovo Cimento
\newcommand{\invp}{Inverse Prob.}        % Inverse problems
\newcommand{\jai}{J.\ Astron.\ Instrumentation} % Journal of Astronomical Instrumentation
\newcommand{\japa}{J.\ Astrophys.\ Astron.} % Journal of Astrophysics and Astronomy
\newcommand{\jastp}{J.\ Atmos.\ Sol.-Terr.\ Phys.} % Journal of Atmospheric and Solar-Terrestrial Physics
\newcommand{\jcap}{J.\ Cosmology Astropart.\ Phys.} % Journal of Cosmology and Astroparticle Physics
\newcommand{\jcomph}{J.\ Comput.\ Phys.} % Journal of Computational Physics
\newcommand{\jcp}{J.\ Chem.\ Phys.}      % Journal of Chemical Physics
\newcommand{\jewa}{J.\ Electromagn.\ Wav.\ Appl.} % Journal of Electromagnetic Waves and Applications
\newcommand{\jgeod}{J.\ Geodesy}         % Journal of Geodesy
\newcommand{\jgr}{J.\ Geophys.\ Res.}    % Journal of Geophysical Research
\newcommand{\jhep}{JHEP}                 % Journal of High Energy Physics
\newcommand{\jinst}{J.\ Instrumentation} % Journal of Instrumentation
\newcommand{\jpsconf}{JPS Conf.\ Proc.}  % Physical Society of Japan Conference Proceedings
\newcommand{\jqsrt}{J.\ Quant.\ Spectrosc.\ Radiative Transfer} % Journal of Quantitative Spectroscopy and Radiative Transfer
\newcommand{\jrasc}{J.\ R.\ Astron.\ Soc.\ Canada} % Journal of the RAS of Canada
\newcommand{\maps}{Meteoritics \& Plan.\ Sci.} % Meteoritics and Planetary Science
\newcommand{\met}{Meteoritics}           % Meteoritics
\newcommand{\memras}{Mem.\ RAS}          % Memoirs of the Royal Astronomical Society
\newcommand{\memsai}{Mem.\ Soc.\ Astron.\ Italiana} % Memorie della Societa Astronomica Italiana
\newcommand{\mnras}{MNRAS}               % Monthly Notices of the RAS
\newcommand{\moonp}{Moon and Plan.}      % Moon and Planets
\newcommand{\mpla}{Mod.\ Phys.\ Lett.~A} % Modern Physics Letters A
\newcommand{\mps}{Meteoritics and Planetary Science} % Meteoritics and Planetary Science
\newcommand{\na}{New Astron.}            % New Astronomy
\newcommand{\nar}{New Astron.\ Rev.}     % New Astronomy Reviews
\newcommand{\nat}{Nature}                % Nature
\newcommand{\nimpr}{Nucl.\ Instrum.\ Meth.\ Phys.\ Res.} % Nuclear Instruments & Methods in Physics Research (prior to section split)
\newcommand{\nima}{Nucl.\ Instrum.\ Meth.~A} % Nuclear Instruments & Methods in Physics Research Section A
\newcommand{\npbproc}{Nucl.\ Phys.~B Proc.\ Supp.} % Nuclear Physics B - Proceedings Supplements
\newcommand{\nphysa}{Nuclear Phys.~A}   % Nuclear Physica A
\newcommand{\njp}{New J.\ Phys.}         % New Journal of Physics
\newcommand{\nspu}{Phys.\ Uspekhi}       % Physics Uspekhi
\newcommand{\pasa}{Publ.\ Astron.\ Soc.\ Australia} % Publications of the Astronomical Society of Australia
\newcommand{\pasj}{PASJ}                 % Publications of the Astronomical Society of Japan
\newcommand{\pasp}{PASP}                 % Publications of the Astronomical Society of the Pacific
\newcommand{\phr}{Phys.\ Rev.}           % Physical Review
\newcommand{\physrep}{Phys.\ Rep.}       % Physics Reports
\newcommand{\physscr}{Phys.\ Scr.}       % Physica Scripta
\newcommand{\physzeit}{Phys.\ Z.}        % Physikalische Zeitschrift
\newcommand{\phss}{Phys.\ Sol.\ Stat.}   % Physics of the Solid State
\newcommand{\pla}{Phys.\ Lett.~A}        % Physics Letters A
\newcommand{\planss}{Planet.\ Space Sci.} % Planetary and Space Science
\newcommand{\plb}{Phys.\ Lett.~B}        % Physics Letters B
\newcommand{\pop}{Phys.\ Plasmas}        % Physics of Plasmas
\newcommand{\pra}{Phys.\ Rev.~A}         % Physical Review A: Atomic, Molecular, and Optical Physics
\newcommand{\prb}{Phys.\ Rev.~B}         % Physical Review B: Solid State
\newcommand{\prc}{Phys.\ Rev.~C}         % Physical Review C: Nuclear Physics
\newcommand{\prd}{Phys.\ Rev.~D}         % Physical Review D: Particles & Fields
\newcommand{\pre}{Phys.\ Rev.~E}         % Physical Review E: Statistical Physics, Plasmas, Fluids, and Related Interdisciplinary Topics
\newcommand{\prl}{Phys.\ Rev.\ Lett.}    % Physical Review Letters
\newcommand{\privcom}{priv.\ comm.}      % private communication
\newcommand{\procsci}{Proc.\ Sci.}       % Proceedings of Science
\newcommand{\procspie}{Proc.\ SPIE}      % Proceedings of the Society of Photo-Optical Instrumentation Engineers
\newcommand{\progpnp}{Prog.\ Part.\ Nucl.\ Phys.} % Progress in Particle and Nuclear Physics
\newcommand{\pst}{Phys.\ Scr.~T}         % Physica Scripta Volume T
\newcommand{\ptep}{Prog.\ Theor.\ Exp.\ Phys.} % Progress of Theoretical and Experimental Physics
\newcommand{\qjras}{QJRAS}               % Quarterly Journal of the RAS
\newcommand{\radres}{Radiation Res.}     % Radiation Research
\newcommand{\radsci}{Radio Sci.}         % Radio Science
\newcommand{\rmxaa}{Rev.\ Mex.\ Astron.\ Astrofis.} % Revista Mexicana de Astronomia y Astrofisica
\newcommand{\rpph}{Rep.\ Prog.\ Phys.}   % Reports on Progress in Physics
\newcommand{\rqe}{Rad.\ \& Quan.\ Elec.} % Radiophysics and Quantum Electronics
\newcommand{\rgsp}{Rev.\ Geophys.\ Space Phys.} % Reviews of Geophysics and Space Physics
\newcommand{\rsla}{Proc.\ R.\ Soc.~A}   % Proceedings of the Royal Society of London Series A: Mathematical, Physical and Engineering Sciences
\newcommand{\sal}{Sov.\ Astron.\ Lett.}  % Soviet Astronomy Letters
\newcommand{\sci}{Science}               % Science
\newcommand{\skytel}{Sky \& Telesc.}     % Sky and Telescope
\newcommand{\solphys}{Sol.\ Phys.}       % Solar Physics
\newcommand{\sovast}{Soviet Ast.}        % Soviet Astronomy
\newcommand{\spjetp}{Sov.\ Phys.\ JETP}  % Soviet Journal of Experimental and Theoretical Physics
\newcommand{\spjetpl}{Sov.\ Phys.\ JETP Lett.} % Soviet Journal of Experimental and Theoretical Physics Letters
\newcommand{\spu}{Sov.\ Phys.\ Usp.}     % Soviet Physics Uspekhi
\newcommand{\ssr}{Space Sci.\ Rev.}      % Space Science Reviews
\newcommand{\yadfiz}{Yad.\ Fiz.}         % Physics of Atomic Nuclei (Yadernaya Fizika)
\newcommand{\zap}{Z.\ Astrophys.}        % Zeitschrift fuer Astrophysik

% Deprecated alternate definitions.
\newcommand{\ajph}{\aujph}
\newcommand{\alet}{\astl}
\newcommand{\applopt}{\ao}
\newcommand{\apjlett}{\apjl}
\newcommand{\apjsupp}{\apjs}
\newcommand{\astap}{\aap}
\newcommand{\nast}{\na}

